Exploring 3D-aware Latent Spaces for Efficiently Learning Numerous Scenes

We present a method enabling the scaling of NeRFs to learn a large number of semantically-similar scenes. We combine two techniques to improve the required training time and memory cost per scene. First, we learn a 3D-aware latent space in which we train Tri-Plane scene representations, hence reducing the resolution at which scenes are learned. Moreover, we present a way to share common information across scenes, hence allowing for a reduction of model complexity to learn a particular scene. Our method reduces effective per-scene memory costs by 44% and per-scene time costs by 86% when training 1000 scenes. Our project page can be found at https://3da-ae.github.io .

==> figures/ae_consistency.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{media/3_method/autoencoder+consistency_fig.png}
    \caption{Illustration of an autoencoder, a latent image and multiview 3d consistency. The desired multiview consistency are highlighted in yellow}
    \label{fig:autoencoder+consistency}
\end{figure}
